Low rank factorization of the Coulomb integrals for periodic coupled cluster theory

We study the decomposition of the Coulomb integrals of periodic systems into a tensor contraction of six matrices of which only two are distinct. We find that the Coulomb integrals can be well approximated in this form already with small matrices compared to the number of real space grid points. The cost of computing the matrices scales as O(N^4) using a regularized form of the alternating least squares algorithm. The studied factorization of the Coulomb integrals can be exploited to reduce the scaling of the computational cost of expensive tensor contractions appearing in the amplitude equations of coupled cluster methods with respect to system size. We apply the developed methodologies to calculate the adsorption energy of a single water molecule on a hexagonal boron nitride monolayer in a plane wave basis set and periodic boundary conditions.

==> TRD-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0.pdf}%
}%
\special{pdf:q}%
\begin{picture}( 240.900000, 150.938232)%
\special{pdf:\ASYraw{
 -240.500000 -0.500000 m
 0.500000 -0.500000 l
 0.500000 150.874328 l
 -240.500000 150.874328 l
 -240.500000 -0.500000 l
h
 -86.094278 72.585814 m
 -8.735281 72.585814 l
 -8.735281 136.858441 l
 -86.094278 136.858441 l
 -86.094278 72.585814 l
h
W* n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-204.833615,27.949711)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-3}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-204.833615,67.262728)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-2}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-204.833615,106.575745)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-204.833615,145.888762)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{0}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-228.544760,86.919237)(-0.500000,0.249999){0.000000 1.000000 -1.000000 0.000000}{\small$|$relative error of MP2$|$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-201.445959,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$0$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-166.455520,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$20$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-131.465082,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$40$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-96.474643,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$60$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-61.484205,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$80$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-26.493766,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$100$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-100.848448,12.355240)(-0.500000,-0.750001){\small number of iterations $I$ ($N_R/N_F=2$)}
\special{pdf:\ASYraw{
 -200.693359 27.845291 m
 -0.250000 27.845291 l
 -0.250000 145.343723 l
 -200.693359 145.343723 l
 -200.693359 27.845291 l
h
W n
}%
}%
\end{picture}%
\kern -240.900000pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{rgb}{1.000000,0.000000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-52.239444,125.700796)(0.000000,-0.500000){\small $N=16$}
\definecolor{ASYcolor}{rgb}{1.000000,0.500000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-52.239444,115.407816)(0.000000,-0.500000){\small $N=24$}
\definecolor{ASYcolor}{rgb}{0.000000,0.500000,0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-52.239444,105.114836)(0.000000,-0.500000){\small $N=36$}
\definecolor{ASYcolor}{rgb}{0.000000,0.000000,1.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-52.239444,94.821856)(0.000000,-0.500000){\small $N=48$}
\definecolor{ASYcolor}{rgb}{0.500000,0.000000,1.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-52.239444,84.528876)(0.000000,-0.500000){\small $N=54$}


==> TRD-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-220.866450,27.949711)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-4}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-220.866450,66.921564)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-3}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-220.866450,105.893418)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-2}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-220.866450,144.865271)(-1.000000,-0.500000){\vphantom{$10^4$}$10^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-217.478793,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-146.158191,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$2$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-74.837588,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$3$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-3.516985,24.562055)(-0.500000,-1.000000){\vphantom{$10^4$}$4$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-110.497889,12.355240)(-0.500000,-0.750001){\small$N_R/N_F$ ($I=120$)}
\special{pdf:q}%
\begin{picture}( 241.265220, 149.914741)%
\special{pdf:\ASYraw{
 -216.666295 27.845291 m
 -3.503846 27.845291 l
 -3.503846 144.324056 l
 -216.666295 144.324056 l
 -216.666295 27.845291 l
h
W n
}%
}%
\end{picture}%
\kern -241.265220pt%
\special{pdf:Q}%


==> TRD-3.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-206.355725,26.177201)(-1.000000,-0.402231){\vphantom{$10^4$}$-70$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,45.365719)(-1.000000,-0.402231){\vphantom{$10^4$}$-60$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,64.554237)(-1.000000,-0.402231){\vphantom{$10^4$}$-50$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,83.742755)(-1.000000,-0.402231){\vphantom{$10^4$}$-40$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,102.931273)(-1.000000,-0.402231){\vphantom{$10^4$}$-30$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,122.119791)(-1.000000,-0.402231){\vphantom{$10^4$}$-20$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,141.308309)(-1.000000,-0.402231){\vphantom{$10^4$}$-10$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.355725,160.496827)(-1.000000,-0.500000){\vphantom{$10^4$}$0$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-227.316940,98.134144)(-0.500000,0.224793){0.000000 1.000000 -1.000000 0.000000}{\small$\epsilon^{\rm OAF}$ [meV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-194.521522,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$750$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-152.288786,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$1000$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-76.269862,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$1450$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-17.144032,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$1800$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-101.609503,10.582730)(-0.500000,-0.815309){\small$N_F$}
\special{pdf:q}%
\begin{picture}( 240.900000, 170.342024)%
\special{pdf:\ASYraw{
 -202.209782 26.079403 m
 -0.250000 26.079403 l
 -0.250000 169.455627 l
 -202.209782 169.455627 l
 -202.209782 26.079403 l
h
W n
}%
}%
\end{picture}%
\kern -240.900000pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-102.201114,65.375329)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$50$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-102.201114,102.089625)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$60$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-115.967929,87.403906)(-0.500000,0.249999){0.000000 1.000000 -1.000000 0.000000}{\small$E_{\rm ads}$ [meV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-94.278058,54.644814)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1589$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-60.291709,54.644814)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$4504$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-16.383445,54.644814)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$8270$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-55.674696,42.437999)(-0.500000,-0.815309){1.000000 0.000000 0.000000 1.000000}{\small$N_G$}
\special{pdf:q}%
\begin{picture}( 240.900000, 170.342024)%
\special{pdf:\ASYraw{
 -98.444291 57.815661 m
 -12.489100 57.815661 l
 -12.489100 116.339071 l
 -98.444291 116.339071 l
 -98.444291 57.815661 l
h
W n
}%
}%
\end{picture}%
\kern -240.900000pt%
\special{pdf:Q}%


==> TRD-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-206.654065,37.690312)(-1.000000,-0.402231){\vphantom{$10^4$}$-16$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.654065,60.716534)(-1.000000,-0.402231){\vphantom{$10^4$}$-12$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.654065,83.742755)(-1.000000,-0.402231){\vphantom{$10^4$}$-8$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.654065,106.768977)(-1.000000,-0.402231){\vphantom{$10^4$}$-4$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.654065,129.795198)(-1.000000,-0.500000){\vphantom{$10^4$}$0$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-206.654065,152.821420)(-1.000000,-0.500000){\vphantom{$10^4$}$4$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-227.615280,98.134144)(-0.500000,0.252082){0.000000 1.000000 -1.000000 0.000000}{\small$\epsilon^{\rm TRD}_{\rm ads}$ [meV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-195.605006,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$1450$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-158.574892,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$2175$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-121.544779,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$2900$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-84.514666,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$3625$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-47.484553,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$4350$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalign(-10.454440,22.789545)(-0.500000,-1.000000){\vphantom{$10^4$}$5075$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-103.668173,10.582730)(-0.500000,-0.815309){\small$N_R$}
\special{pdf:q}%
\begin{picture}( 241.642660, 170.342024)%
\special{pdf:\ASYraw{
 -202.507007 26.079403 m
 -4.054732 26.079403 l
 -4.054732 169.455627 l
 -202.507007 169.455627 l
 -202.507007 26.079403 l
h
W n
}%
}%
\end{picture}%
\kern -241.642660pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-95.674606,51.641337)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-95.674606,81.756764)(-1.000000,-0.500000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$10^{2}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalignT(-113.608031,73.432228)(-0.500000,0.308114){0.000000 1.000000 -1.000000 0.000000}{\small$\epsilon^{\rm TRD}_{\rm H_2O+BN}$ [meV]}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-88.149023,43.588742)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$1450$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.033750}{10.840500}\selectfont
\ASYalignT(-28.149081,43.588742)(-0.500000,-1.000000){1.000000 0.000000 0.000000 1.000000}{\vphantom{$10^4$}$5075$}
\special{pdf:q}%
\begin{picture}( 241.642660, 170.342024)%
\special{pdf:\ASYraw{
 -91.942167 46.800895 m
 -24.333695 46.800895 l
 -24.333695 99.514877 l
 -91.942167 99.514877 l
 -91.942167 46.800895 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{11.041250}{13.249500}\selectfont
\ASYalign(-58.355948,86.667619)(-0.500000,0.068964){\small$0.1\%$}
\end{picture}%
\kern -241.642660pt%
\special{pdf:Q}%

